Systematic Evaluation of Neural Retrieval Models on the Touch\'e 2020 Argument Retrieval Subset of BEIR

The zero-shot effectiveness of neural retrieval models is often evaluated on the BEIR benchmark -- a combination of different IR evaluation datasets. Interestingly, previous studies found that particularly on the BEIR subset Touch\'e 2020, an argument retrieval task, neural retrieval models are considerably less effective than BM25. Still, so far, no further investigation has been conducted on what makes argument retrieval so "special". To more deeply analyze the respective potential limits of neural retrieval models, we run a reproducibility study on the Touch\'e 2020 data. In our study, we focus on two experiments: (i) a black-box evaluation (i.e., no model retraining), incorporating a theoretical exploration using retrieval axioms, and (ii) a data denoising evaluation involving post-hoc relevance judgments. Our black-box evaluation reveals an inherent bias of neural models towards retrieving short passages from the Touch\'e 2020 data, and we also find that quite a few of the neural models' results are unjudged in the Touch\'e 2020 data. As many of the short Touch\'e passages are not argumentative and thus non-relevant per se, and as the missing judgments complicate fair comparison, we denoise the Touch\'e 2020 data by excluding very short passages (less than 20 words) and by augmenting the unjudged data with post-hoc judgments following the Touch\'e guidelines. On the denoised data, the effectiveness of the neural models improves by up to 0.52 in nDCG@10, but BM25 is still more effective. Our code and the augmented Touch\'e 2020 dataset are available at \url{https://github.com/castorini/touche-error-analysis}.

==> tables/summarized-argument-example.tex <==

\begin{table*}[t]
    \centering
    \scriptsize
    \begin{tabular}{p{1.8cm}|p{10.2cm}}
    \toprule
    \multicolumn{2}{l}{Touch{\'e}~2020 Query: Can alternative energy effectively replace fossil fuels?} \\ \midrule
    \textbf{Original} & $<$fossil fuel$>$ Unlike what my opponent argues, there are many alternatives to fossil fuel. fossil fuel is just a way to draw energy from the earth. some of these alternatives are Nuclear fusion geothermal energy wind and solar power Going back to my first alternative, nuclear fusion. Nuclear fusion is a very effective way for one to create a mass amount of energy ... \\ \midrule
    \cellcolor{green!20}\textbf{GPT-3.5 Summary} & \cellcolor{green!20}The argument presented is that there are many alternatives to fossil fuel and that these alternatives, such as nuclear fusion, geothermal energy, and solar and wind power, are both efficient and cost-effective. The argument emphasizes the need for a new and better source of energy ... \\ \midrule
    \cellcolor{green!20}\textbf{DocT5query (10 questions)} & \cellcolor{green!20}what is the alternative to fossil fuels for energy? what is one alternative energy source? what is an alternative energy source for fossil fuels? what is the difference between fossil fuels and geothermal energy? why are nuclear fusion used in energy production? how much energy do fossil fuels generate? ... \\ 
    \bottomrule
    \end{tabular}
    \caption{Query, Relevant Document, GPT-3.5 Summary and DocT5Query-generated queries for an example from Touch{\'e}~2020.}
    \label{tab:retrieval-documents-examples}
\end{table*}
